Why This and Not That? A Collaborative Reflection Approach for Understanding Thought Coverage in Decision Making Support Dialog

Conversational agents that support reflection for decision-making often rely on adaptive dialog policies that map observed user behavior to actions such as probing, deepening, or redirecting. Yet the same pattern can reflect a range of different reasons such as deliberate prioritisation or limited self-access. By modeling the observable pattern rather than the user's reason for it, current policies risk premature assumptions about the user state and inappropriate next actions. To address this gap, we introduce a human-centered method for surfacing this hidden inference step. In a user study with 62 users and 232 collaborative moments, we pause a reflection-support agent when it would normally redirect the conversation, surface its observation, and ask users to interpret the pattern and decide how to proceed. We derive a taxonomy of nine interpretation categories and show that similar reflective states can call for substantially different follow-up actions. Our findings challenge the assumption that adaptive dialog policies can rely on observable behavior alone, and suggest how user-provided interpretations can inform more appropriate conversational actions.

==> method-p3.tex <==
\subsubsection{Procedure}
The study was conducted on a web-based platform. After reviewing and agreeing to an informed consent form outlining the study purpose, data usage, and participant rights, participants completed a pre-study questionnaire collecting demographic information as well as the short form of the Self-Reflection and Insight Scale (SRIS)~\cite{SRIS-short}.
Participants then selected a decision topic and entered the “unaided reflection” phase, during which they freely wrote down their thoughts without any agent support. Once they indicated that they had no further thoughts to add, they proceeded to an “assisted reflection” phase, in which they interacted with the conversational agent. This interaction continued until participants chose to end the session.


\subsection{Participants}
We recruited 62 participants via the crowd-sourcing platform Prolific\footnote{\url{https://www.prolific.com}}.
Inclusion criteria were fluency in English and currently being in the process of making one of the big life decisions~\cite{camilleri2023investigation} listed in Appendix-F. 

The sample was diverse in terms of age (M = 34.27, SD = 8.66, median = 30, range 21–60), gender (30 female, 32 male), education level (ranging from high school to doctoral degrees), self-insight scores (M = 26.55, SD = 6.22, median = 26), and selected decision topics.



==> method.tex <==
\subsection{The Reflection Agent}
 
We build on ReflectiMate~\cite{reflectimate}, a reflection-support agent that maintains a structured knowledge base (KB) of the user's thoughts, organised into three categories: \textit{internal} (feelings, values, emotions), \textit{external} (practical constraints, other people, real-world conditions), and \textit{experiential} (past experiences, lessons from others). The agent tracks two dimensions per category: \textit{breadth} (number of distinct thoughts) and \textit{depth} (degree of elaboration per thought), updated after each conversational turn.
 
The agent's policy pursues two objectives: (1)~disrupting fixation patterns by redirecting attention to underexplored categories, and (2)~disrupting shallow reasoning by prompting deeper elaboration on underdeveloped thoughts. The agent makes these strategic decisions through a fixed pipeline: it observes a pattern in the KB, applies an interpretation, and decides on the next action. Specifically, when the agent detects asymmetry in a cumulative coverage indicator across categories, it uniformly interprets this as the user fixating and decides to switch the conversation to the lowest-scoring category.
 
\subsection{The Experimental Protocol}
 
Rather than acting on its interpretation silently, the experimental agent pauses the conversation at every point where it would switch categories and presents a three-step protocol in a visually separate side panel:
 
\paragraph{Step 1 --- Recognition.} The agent surfaces its observation and asks: \textit{``Do you recognise this pattern in your reflection?''} If the user says no, they describe what they see instead.
 
\paragraph{Step 2 --- Interpretation.} The agent asks: \textit{``Do you have a feeling for why that could be?''} The user provides their reason in an open text field.
 
\paragraph{Step 3 --- Decision.} The agent asks: \textit{``What would you like to explore next?''} The user selects from dynamically generated options corresponding to the available categories and provides their reasoning. An optional field asks whether any action was missing from the options.
 
The observation text adapts to the KB state. When a cross-category mismatch is detected (the user was directed toward one category but responses gravitated to another), the observation surfaces this. When the dominant category is one the user previously chose, the observation acknowledges this and points to what remains uncovered. Otherwise, the observation describes the coverage distribution directly. The agent never reveals its default interpretation or decision. The protocol was validated through expert review and a pilot study with five participants using cognitive interviewing~\cite{willis2004cognitive}.
 
Each collaborative moment produces a logged data tuple: the KB state at trigger time, the agent's default interpretation and decision (logged but not shown), the observation text, the user's recognition response, interpretation, decision, and reasoning.
 
\subsection{Data Collection}
 
\paragraph{Participants.} We recruited $N$ participants via Prolific, each reflecting on a real pending personal decision from from a predefined list of big life decisions \cite{camilleri2023investigation} (e.g., career changes, financial decisions, relationship decisions). 
Inclusion criteria required participants to be currently in the process of making one of these decisions and to be fluent in English. 


 
\paragraph{Procedure.} After informed consent and the pre-questionnaire, where  all participants completed the Self-Reflection and Insight Scale (SRIS-S;~\cite{silvia2022self}) and a brief demographic survey, the session proceeds in two phases. 
In the unaided phase, participants wrote freely about their decision for as long as they wish.  
In the assisted phase, the agent engaged them in a structured conversation, pausing at every category-switching moment to present the three-step protocol. %After the conversation, participants completed a brief questionnaire.

\subsection{Analysis}

\subsubsection{Taxonomy Building (RQ1)}

A human coder (the primary researcher) manually coded all interpretation responses using an inductive qualitative analysis process. Coding order was determined through maximum variation sampling~\cite{patton2014qualitative} based on SRIS-S insight scores, ensuring that the initial codebook was constructed from participants with diverse self-reflective tendencies. Initial coding began with six participants drawn from the extremes of the insight score distribution.

For each interpretation response, the coder reviewed the full context --- including the observation text, the user's recognition response, and the interpretation response --- assigned a code, and wrote an analytic memo documenting the rationale for the assignment. After each batch of six participants, codes were grouped into candidate categories with accompanying definitions, inclusion and exclusion criteria, and prototypical examples. Categories were iteratively refined through constant comparison with newly coded data. Code saturation was monitored following~\citet{hennink2017code} and was considered reached once six consecutive participants yielded no new categories.

\paragraph{Inter-rater reliability.} 
After completion of the coding process, we assessed inter-rater reliability using local language models as independent coders, following recent work demonstrating the validity of LLM-based reliability assessment for qualitative coding~\cite{jain2026multillm}. We evaluated models from four families (Qwen 2.5~\citep{}, Mistral~\citep{}, Phi-4~\citep{}, and Gemma 2~\citep{}) across two prompt designs (Appendix~B). Using models from different families provided more independent classifications, as models within the same family may share training biases that could artificially inflate agreement~\cite{than2025updating}. Each model independently classified all responses against the final codebook without access to the researcher’s annotations. All language models were run locally via Ollama to ensure that participant data remained on secure servers.


\subsubsection{Alignment Analysis (RQ2)}
 
For each collaborative moment, the user's chosen action is compared against the agent's logged default. We compute alignment rates overall and per taxonomy category, and examine user choice distributions within each dominant state to assess whether the taxonomy category mediates between the observable state and the user's chosen direction. To characterise the nature of divergence, we classify each user choice as moving toward an underexplored dimension or staying with the dominant one, and report these rates overall and by taxonomy category.
 
